The virtual element method for resistive magnetohydrodynamics

We present a virtual element method (VEM) for the numerical approximation of the electromagnetics subsystem of the resistive magnetohydrodynamics (MHD) model in two spatial dimensions. The major advantages of the virtual element method include great flexibility of polygonal meshes and automatic divergence-free constraint on the magnetic flux field. In this work, we rigorously prove the well-posedness of the method and the solenoidal nature of the discrete magnetic flux field. We also derive stability energy estimates. The design of the method includes three choices for the construction of the nodal mass matrix and criteria to more alternative. We present a set of numerical experiments that independently validate theoretical results. The numerical experiments include the convergence rate study, energy estimates and verification of the divergence-free condition on the magnetic flux field. All these numerical experiments have been performed on triangular, perturbed quadrilateral and Voronoi meshes. Finally, We demonstrate the development of the VEM method on a numerical model for the Hartmann flow.

==> introVEM.tex <==
\subsection{Background material on the VEM}

The VEM was originally proposed as a reformulation in a variational
setting of the \emph{nodal} mimetic finite difference (MFD)
method~\cite{% 
BeiraodaVeiga-Manzini-Putti:2015,%
BeiraodaVeiga-Lipnikov-Manzini:2011,% 
Brezzi-Buffa-Lipnikov:2009,%
Manzini-Lipnikov-Moulton-Shashkov:2017% 
} 
for the numerical treatment of elliptic problems on unstructured
polygonal and polyhedral meshes.
%%
The research monograph~\cite{BeiraodaVeiga-Lipnikov-Manzini:2014}.
and the survey paper~\cite{Lipnikov-Manzini-Shashkov:2014} offers a
detailed review of the MFD method.
%% 
The main feature of the MFD method, i.e., its great flexibility with
respect to the admissible meshes used in the numerical formulation,
are inherited by the VEM.
%%
Moreover, the variational formulation makes it possible to exploit all
the functional tools that are normally used in the analysis of the
finite element method, to prove the converge of the VEM approximation and 
derive error estimates.
%%
These facts have dsetermined the success of the VEM, as is
reflected in the numerous 
applications developed in the last few years, see, for
example,~\cite{%
Antonietti-BeiraodaVeiga-Scacchi-Verani:2016,%
Cangiani-Georgoulis-Pryer-Sutton:2016,%
BeiraodaVeiga-Lovadina-Vacca:2016,%
BeiraodaVeiga-Chernov-Mascotto-Russo:2016,%
BeiraodaVeiga-Brezzi-Marini-Russo:2016a,%
BeiraodaVeiga-Brezzi-Marini-Russo:2016b,%
BeiraodaVeiga-Brezzi-Marini-Russo:2016c,%
BeiraodaVeiga-Brezzi-Marini-Russo:2016d,%
Benedetto-Berrone-Borio-Pieraccini-Scialo:2016b,%
Berrone-Borio-Scialo:2016,Benedetto-Berrone-Scialo:2016,%
Berrone-Pieraccini-Scialo:2016,Perugia-Pietra-Russo:2016,%
Wriggers-Rust-Reddy:2016,BeiraodaVeiga-Lovadina-Mora:2015,%
BeiraodaVeiga-Manzini:2015,Mora-Rivera-Rodriguez:2015,%
Natarajan-Bordas-Ooi:2015,Berrone-Pieraccini-Scialo-Vicini:2015,%
Vacca-BeiraodaVeiga:2015,Paulino-Gain:2015,%
Antonietti-BeiraodaVeiga-Mora-Verani:2014,%
BeiraodaVeiga-Brezzi-Marini-Russo:2014,%
BeiraodaVeiga-Brezzi-Marini-Russo:2014b,BeiraodaVeiga-Manzini:2014,%
Benedetto-Berrone-Pieraccini-Scialo:2014,%
BeiraodaVeiga-Brezzi-Marini:2013,Brezzi-Marini:2013,%
Berrone-Benedetto-Borio:2016chapter,Berrone-Borio:2017,%
Benedetto-Berrone-Borio-Pieraccini-Scialo:2016eccomas,%
Benvenuti-Chiozzi-Manzini-Sukumar:2019:CMAME:journal,%
Antonietti-Manzini-Verani:2019:CAMWA:journal,%%
Certik-Gardini-Manzini-Mascotto-Vacca:2019:CAMWA:journal,%
Certik-Gardini-Manzini-Vacca:2018:ApplMath:journal,%%
BeiraodaVeiga:2019:NumerMath:journal}.
%% 
The VEM has strong similarities with other numerical formulations, as
pointed out
in~\cite{Manzini-Russo-Sukumar:2014,Cangiani-Manzini-Russo-Sukumar:2015,DiPietro-Droniou-Manzini:2018}
concerning finite elements on polygonal/polyhedral meshes ,
in~\cite{DiPietro-Droniou-Manzini:2018:JCP:journal} concerning
discontinuous skeletal gradient discretizations,
in~\cite{Cangiani-Gyrya-Manzini-Sutton:2017:GBC:chbook} concerning the
BEM-based FEM method.

\medskip
%%
The VEM was originally formulated
in~\cite{BeiraodaVeiga-Brezzi-Cangiani-Manzini-Marini-Russo:2013} as a
conforming FEM for the Poisson problem.
%%
It was later extended to convection-reaction-diffusion problems with
variable coefficients
in~\cite{Ahmad-Alsaedi-Brezzi-Marini-Russo:2013,BeiraodaVeiga-Brezzi-Marini-Russo:2016b}.
%%
Meanwhile, the nonconforming formulation for diffusion problems was
proposed in~\cite{AyusodeDios-Lipnikov-Manzini:2016} as the finite
element reformulation of~\cite{Lipnikov-Manzini:2014} and later
extended to general elliptic
problems~\cite{Cangiani-Manzini-Sutton:2017,Berrone-Borio-Manzini:2018:CMAME:journal}, Stokes
problem~\cite{Cangiani-Gyrya-Manzini:2016}, 
eigenvalue problems~\cite{Gardini-Manzini-Vacca:2019:M2AN:journal},
and the biharmonic
equation~\cite{Antonietti-Manzini-Verani:2018,Zhao-Chen-Zhang:2016}.

\medskip
%%
Mixed VEM for elliptic problems were introduced
in~\cite{Brezzi-Falk-Marini:2014} in a BDM-like setting and further
developed in~\cite{BeiraodaVeiga-Brezzi-Marini-Russo:2016c} in an
RT-like setting.
%% 
Furthermore, 



==> mydefs.tex <==
%% macros for text redaction
\newcommand{\EOD}{\end{document}} 
\newcommand{\TBW}{\textbf{To be written\ldots}}
\newcommand{\BIB}{[\textbf{BIB}]}
\newcommand{\CITE}[1]{[\textbf{Cite~#1}]}
\newcommand{\FNOTE}[1]{\footnote{\textbf{#1}}}

%%%%%Environments
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{remark}{Remark}
\newtheorem{definition}{Definition}
\newtheorem{Proposition}{Proposition}
\newtheorem{proof}{Proof}

%% functional spaces
\newcommand{\CS}[1]{C^{#1}}
\newcommand{\HS}[1]{H^{#1}}
\newcommand{\PS}[1]{\mathbbm{P}_{#1}}
\newcommand{\LTWO}{L^2}
\newcommand{\LINF}{L^{\infty}}

%% norm & semi-norm symbols
\newcommand{\norm} [2]{|\!|#1|\!|_{#2}}
\newcommand{\snorm}[2]{|#1|_{#2}}

%% ----------------------------------

\newcommand{\calE}{\mathcal{E}}
\newcommand{\calM}{\mathcal{M}}

%% ----------------------------------

%% Mesh symbols
\newcommand{\Th}{\Omega_h}
\newcommand{\hh}{h}
\newcommand{\xs}{x}

%% sets
\newcommand{\Pset}{\mathcal{P}}    % mesh polyhedrons
\newcommand{\Fset}{\mathcal{F}}    % mesh faces
\newcommand{\Eset}{\mathcal{E}}    % mesh edges
\newcommand{\Vset}{\mathcal{V}}    % mesh nodes
\newcommand{\Sset}{\mathcal{S}}    % generic symbol

%% ----------------------------------

%% generic math symbols
\newcommand{\KER} {\textrm{ker}}
\newcommand{\INTP}{\footnotesize{I}}
\newcommand{\SPAN}[1]{\mbox{\textrm{span}}\big\{#1\big\}}
\newcommand{\REAL}{\mathbbm{R}}
\newcommand{\INTG}{\mathbbm{N}}
\newcommand{\CARD}[1]{\#{\left(#1\right)}}
\newcommand{\ASSUM}[1]{\textbf{(#1)}}

%% general
\newcommand{\DIM} {d}              % space dimension
\newcommand{\INT} {0}              % internal objects
\newcommand{\BND} {\partial}       % boundary objects

%% ----------------------------------

\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bbc}{\mathbf{c}}
\newcommand{\bd}{\mathbf{d}}
%% ---
\newcommand{\be}{\mathbf{e}}
\newcommand{\bbf}{\mathbf{f}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bh}{\mathbf{h}}
%% ---
\newcommand{\bi}{\mathbf{i}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bc}{\mathbf{k}}
\newcommand{\bl}{\mathbf{l}}
%% ---
\newcommand{\bbm}{\mathbf{m}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bp}{\mathbf{p}}
%% ---
\newcommand{\bq}{\mathbf{q}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bt}{\mathbf{t}}
%% ---
%% \newcommand{\bu}{\mathbf{u}} %% defined in preamble.tex
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
%% ---
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}

%% ----------------------------------

\newcommand{\vs}{v}

==> sec_6_numerical-old.tex <==
\section{Numerical experiments}
\label{Sec:NumericalExperiments}

In this section we will summarize a series of numerical experiments that sheds some light on the performance of the VEM developed and analyzed throughout this article. It is divided in three sections, the first on explores the rate of convergence and the divergence preserving nature of the numerical method. The second section studies the energy estimate that was introduced in theorem \ref{theorem:DiscreteEnergyEstimate}. The final section we introduce the Hartmann problem and use this novel discretization to approximate its solution.
% \subsection*{\textbf{General comments}}

% \begin{itemize}
% \item I removed the tables because they are not very informative
%   (nobody wants to look at list of numbers) and they do not provide
%   more information than plots, which are, in general, much easier to
%   read and understand

%   \medskip
% \item in all plots, please remove the labels. It is much better to
%   manage them directly from latex. Also, use thicker lines and
%   markers. It is not specified if errors are \emph{relative} or
%   \emph{absolute}
%   %% 
%   It is better to show \textbf{relative errors}, so if you show
%   absolute errors, please, can you fix them?
  
%   \medskip
% \item also, do not use colors to distinguish things unless you want to
%   pay the journal to print colored pages.

%   \medskip
% \item in the first example, it may make sense to show a comparison of
%   the performance of the different version that we can have by
%   changing the pseudo-projection operator $\PiVhP$ according to the
%   discussion in section~3.

%   \medskip
% \item in the second example, please, provide (as commented) more
%   explanations on why this example is important in general and why VEM
%   are a good choice for it

%   \medskip
% \item I think that this section must be strengthen a bit more. I
%   suggest to consider at least a third example taken from the MHD
%   literature.
% \end{itemize}

\subsection{Experimental analysis of the rate of convergence and the divergence free condition.}
%%

To assess the performance of the VEM we study the numerical approximations of
Problem~\ref{eq:VarForEq2} on $\Omega=[-1,1]^2$.
%%
To this end, we consider the velocity field $\uv=(\us_x,\us_y)^T$ given by
\begin{align}
  \us_x(x,y)&=-\frac{(x^2+y^2-1)(\sin(xy)+\cos(xy))-100e^{x}+100e^{y}}{2(50e^x-y\sin(xy)+y\cos(xy))},\\[0.25em]
  \us_y(x,y)&=\frac{(x^2+y^2-1)(\sin(xy)+\cos(xy))-100e^{x}+100e^{y}}{2(50e^y+x\sin(xy)-x\cos(xy))}.
\end{align}
and initial and boundary conditions are set in accordance with the exact solution electromagnetic fields:
\begin{align}
  \Bv(x,y,t) &= 
  \begin{pmatrix}
    50e^y+x\sin(xy)-x\cos(xy)\\[0.25em]
    50 e^x-y\sin(xy)+y\cos(xy)
  \end{pmatrix}e^{-t},\\[0.5em]
  \Es(x,y,t) &= -\big( 50(e^x-e^y)+\cos(xy)+\sin(xy) \big) e^{-t}.
\end{align}
% 
To check the robustness of the method we have selected three different
mesh families, including triangular meshes, randomly perturbed square
meshes, and meshes based on Voronoi tessellations.
%%
A example of each mesh family is shown in Figure~\ref{fig:Meshes}.

\begin{figure}[t!]
  \begin{center} 
    \includegraphics[width=.30\textwidth]{./figures/TriangularMesh.eps} \hspace{2mm}
    \includegraphics[width=.30\textwidth]{./figures/PerturbedSquaresMesh.eps}\hspace{2mm}
    \includegraphics[width=.30\textwidth]{./figures/VoronoiMesh.eps}
    \caption{Illustration of the meshes used for testing the rate of
      convergence: triangular mesh (left panel), perturbed square mesh
      (central panel) and Voronoi tesselation (right panel).}
    \label{fig:Meshes}
  \end{center}
\end{figure}


The time marching scheme uses $\theta =1/2$, errors with different values of $\theta$ are very similar and thus we omit them.  
%%
The final time is set at $T=0.25$ and the timestep follows the
assignment $\Dt=0.05\hh^2$.
%% 
Figure~\ref{fig:test1:convergence-curves} shows the log-log plots of
the error curves on the approximation of the electric and magnetic
fields.
%%
The errors are measured in the $\LTWO$ norms.

An important feature of the VEM we present is that the magnetic field remains divergence free throughout the simulations. 
%
Next, we will present the results numerical experiments aimed at gathering experimental evidence towards to support the theoretical findings.
%
In Figure~\ref{fig:DivPlots} we present three simulations, each done in a different type of mesh, the $y-$axis represents the squared $L^2$ norm of the magnetic field.

subsection{Experimental analysis of the energy estimates}

This section is dedicated to an experimental study of the energy estimate presented in 
theorem \ref{theorem:DiscreteEnergyEstimate}.
%
For this purpose we define a normalized version of the right hand side, the left hand side of \eqref{eq:DiscEstTwo} and their difference as:
%
\begin{align}
    &\calE_R(n) = \frac{\TNORM{\Bvh^{0}}{\Eh}^2 +
      \gamma\Dt\sum_{\ell=0}^{n}\beta^{n+1-\ell}
      \TNORM{\IVh\Es_0^{n-\ell+\theta}}{\HROTv{\Omega}}^2}{\TNORM{\Bvh^{0}}{\Eh}^2}, 
      \\
    &\calE_L(n) = \frac{(\beta)^{n+1}\TNORM{\Bvh^{n+1}}{\Eh}^2 
      +\frac{\gamma\Dt}{2}\sum_{\ell=0}^{n}\beta^{n+1-\ell}\TNORM{\hEsh^{n-\ell+\theta}}{\Vh}^2}{\TNORM{\Bvh^{0}}{\Eh}^2},
      \\
    &\calE(n) = \calE(n)_R-\calE_L(n).
\end{align}
%
Notice that, by hypothesis \eqref{eq:Assumption}, the value of $\beta$ as defined in \eqref{eq:beta-Q:def} is necessarily smaller than $1$, which implies that most of the coefficients in the terms that appear in $\calE$ decay exponentially. Therefore, we can expect that $\calE\to 1$ as $n\to\infty$ unless the growth, in time, of the electric and magnetic fields is fast enough to offset this decay. To exemplify this we introduce the parameter $C\in\mathbbm{R}$ and the family of solutions
%
\begin{align}
\Bv^C(x,y,t) &= 
  \begin{pmatrix}
    50e^y-x\sin(xy)+x\cos(xy)\\[0.25em]
    50 e^x+y\sin(xy)+y\cos(xy)
  \end{pmatrix}e^{Ct},\\
  \Es^C(x,y,t) &= C\big( 50(e^x-e^y)-\cos(xy)-\sin(xy) \big) e^{Ct}.
\end{align}
%
and velocity fields $\uv^C=(\us_x^C,\us_y^C)^T$ for
\begin{align}
  \us_x^C(x,y)&=-C\frac{(-x^2-y^2-1)(\sin(xy)+\cos(xy))}{2(50e^x+y\sin(xy)-y\cos(xy))},\\[0.25em]
  \us_y^C(x,y)&=C\frac{(-x^2-y^2-1)(\sin(xy)+\cos(xy))}{2(50e^y-x\sin(xy)+x\cos(xy))}.
\end{align}
%
as well as conductivity $\sigma\equiv 1/C$.


%%   TEST CASE: MANUFACTURED SOLUTION 
%%
\begin{figure}[H]
  \begin{center}
    \begin{tabular}{cc}
      %% TRIANGULAR MESHES
      \begin{overpic}[width=.475\textwidth]{./figures/ElectricTriangularConvergence.eps}
       \put( 0,8.5){\begin{sideways}\textbf{Electric field relative error}\end{sideways}}
        \put(40,-2){\textbf{Mesh size $\mathbf{h}$}}
        \put(17,29){\textbf{2}}
        \put(26,36){\textbf{1}}
      \end{overpic}
      & \qquad
      \begin{overpic}[width=.475\textwidth]{./figures/MagneticTriangularConvergence.eps}
       \put( 0,7.5){\begin{sideways}\textbf{Magnetic field relative error}\end{sideways}}
        \put(40,-2) {\textbf{Mesh size $\mathbf{h}$}}
        \put(17,29){\textbf{1}}
        \put(25,38){\textbf{1}}
      \end{overpic}
      %\\[1.em]
      %% OLD \includegraphics[width=.4\textwidth]{./figures/ElectricTriangularConvergence.png} &\qquad
      %% OLD \includegraphics[width=.4\textwidth]{./figures/MagneticTriangularConvergence.png} \\[0.25em]
      %\multicolumn{2}{c}{$(a)$ Error curves for triangular meshes}
      \vspace{-5mm} \\[1.5em] 
      %% ----------------------------------------------------------------------
      %% QUAD MESHES
      \begin{overpic}[width=.475\textwidth]{./figures/ElectricQuadConvergence.eps}
       \put( 0,8.5){\begin{sideways}\textbf{Electric field relative error}\end{sideways}}
        \put(40,-2) {\textbf{Mesh size $\mathbf{h}$}}
        \put(16,34){\textbf{2}}
        \put(25,42){\textbf{1}}
      \end{overpic}
      & \qquad
      \begin{overpic}[width=.475\textwidth]{./figures/MagneticQuadConvergence.eps}
       \put( 0,7.5){\begin{sideways}\textbf{Magnetic field relative error}\end{sideways}}
        \put(45,-2) {\textbf{Mesh size $\mathbf{h}$}}
        \put(16,25){\textbf{1}}
        \put(25,32){\textbf{1}}
      \end{overpic}
      %\\[1.em]
      %% OLD \includegraphics[width=.4\textwidth]{./figures/ElectricQuadConvergence.png} &\qquad
      %% OLD \includegraphics[width=.4\textwidth]{./figures/MagneticQuadConvergence.png} \\[0.25em]
      %\multicolumn{2}{c}{$(b)$ Error curves for perturbed square meshes} 
      \vspace{-5mm} \\[1.5em] 
      %% ----------------------------------------------------------------------
      %% VORONOI MESHES
      \begin{overpic}[width=.475\textwidth]{./figures/ElectricVoronoiConvergence.eps}
       \put( 0,8.5){\begin{sideways}\textbf{Electric field relative error}\end{sideways}}
        \put(40,-2) {\textbf{Mesh size $\mathbf{h}$}}
        \put(15,40){\textbf{2}}
        \put(23,47){\textbf{1}}
      \end{overpic}
      & \qquad
      \begin{overpic}[width=.475\textwidth]{./figures/MagneticVoronoiConvergence.eps}
       \put( 0,7.5){\begin{sideways}\textbf{Magnetic field relative error}\end{sideways}}
        \put(40,-2) {\textbf{Mesh size $\mathbf{h}$}}
        \put(14,25){\textbf{1}}
        \put(23,33){\textbf{1}}
      \end{overpic}
      %\\[1.5em]
      %% OLD \includegraphics[width=.4\textwidth]{./figures/ElectricVoronoiConvergence.png} &\qquad
      %% OLD \includegraphics[width=.4\textwidth]{./figures/MagneticVoronoiConvergence.png} \\[0.25em]
      %\multicolumn{2}{c}{$(c)$ Error curves for Voronoi tesselations.}
    \end{tabular}
  \end{center}
  
  \medskip
 \caption{ Error curves for the virtual element approximation of the electric and magnetic field (respectively, left and right panels)
    on the three mesh families of Figure~\ref{fig:Meshes}: triangular mesh family (top), quadrilateral mesh family (middle), Voronoi mesh family (bottom).
    %% 
    The convergence rate is reflected by the slope of the curves in
    the log-log plots; the reference convergence is shown by the
    triangle in each plot. The symbols E,LS,GI refers to the three alternatives we have for constructing the nodal mass matrix the elliptic projector, least squares projector and the Galerkin interpolator respectively.}
  \label{fig:test1:convergence-curves}
\end{figure}

\begin{figure}[H]
  \begin{center}
    \begin{tabular}{ccc}
      %% Triangular Mesh
      \begin{overpic}[width=.3\textwidth]{./figures/TriangularDivplot.eps}
        \put(45,-2){{\small\textbf{Time}}}
      \end{overpic}
      & \qquad
      %%Quadrilateral Mesh
      \begin{overpic}[width=.3\textwidth]{./figures/QuadDivplot.eps}
        \put(45,-2){{\small\textbf{Time}}}
      \end{overpic}
      &\qquad
      %%Voronoi Mesh
      \begin{overpic}[width=.3\textwidth]{./figures/VoronoiDivplot.eps}
        \put(45,-2){{\small\textbf{Time}}}
      \end{overpic}
     \end{tabular}
  \end{center}
  \label{fig:DivPlots}
  \caption{Plots of the time evolution of the square $L^2$ norm of the divergence of the numerical magnetic field on the three mesh families of figure~\ref{fig:Meshes}. The top left in a triangular mesh, the top right is in a mesh with quadrilateral cells and finally the bottom summarizes the results in a Voronoi tesselation.}
  %Mesh sizes Trig = 0.051886, quad = 0.043478, Vor = 0.0677285
\end{figure}

\




Note that the hypothesis  yields that any choice of $0<Q<\theta^{-1}$, as defined in \eqref{eq:beta-Q:def}, is admissible.
%
In figure~\ref{fig:QvsEnergy} we plot difference between the right and left hand sides of \eqref{eq:DiscEstTwo} normalized by the squared $L^2$-norm of the initial condition on the magnetic field against the value of $Q$ at time $T=0.5$.
%
The type of mesh or the alternative on the nodal mass matrix do not yield significant difference on figure.
%
Thus, we present the results on Voronoi tessalations of the elliptic projector as a representative of all of them, the mesh size is $h=0.0678$.
%
\begin{figure}[H]
  \begin{center}
    \begin{tabular}{cc}
      \begin{overpic}[width=.475\textwidth]{./figures/QvsEnergysmallC.eps}
       \put( 1,35){\begin{sideways}\textbf{$\calE$}\end{sideways}}
        \put(50,0){\textbf{Q}}
      \end{overpic}
      \qquad
    \begin{overpic}[width=.475\textwidth]{./figures/QvsEnergylargeC.eps}
       \put( 1,35){\begin{sideways}\textbf{$\calE$}\end{sideways}}
        \put(50,0){\textbf{Q}}
      \end{overpic}
     \end{tabular}
  \end{center}
  \label{fig:QvsEnergy}
  \caption{Plot of Q against the resulting energy estimate. The initial data that yields the plot in the left is that associated with $C = 0.1$ and time step $\Dt=0.001$, whereas the results on the right figure are associated with $C = 5$ and $\Dt=0.21$}
\end{figure}

The results of figure \ref{fig:QvsEnergy} are simple to explain. 
%
In the case that the growth of the solution is relatively small only the values of $Q$ near that yield $\beta\approx 1$ and the coefficients in $\calE$ will show some exponential growth, if $Q\approx \theta^{-1}$ then the value of $\gamma$ blows up yielding that $\calE$ will be large.
%
The rest of the values of $Q$ will show convergence towards the norm of the initial conditions on the magnetic field, since we normalized by this value we can expect a flat line of height one.
%
If, however, the solution grows faster than the decay brought about by the coefficients in $\calE$ then we will see the energy blow up.
%
Note that the growth in time, at least in out example, of $\calE$ is mainly ruled by terms that look like $\beta^{n} e^{C\Dt n}$ were $t= n\Dt$, hence a rule of thumb for checking whether the energy will grow or flatten is to check if $\ln{\beta}+C\Dt$ is positive or negative respectively.
%
This is the reason we picked such a small value for $\Dt$ in the right plot of figure \ref{fig:QvsEnergy} since large values of $C$ can yield overflow errors.
%
In figure \ref{fig:EnergyEstimates} we can clearly see the two different types of behavior that the energy estimates present.
\begin{figure}[H]
  \begin{center}
    \begin{tabular}{cc}
      %%beta<<1
      \begin{overpic}[width=.475\textwidth]{./figures/EnergyDecay.eps}
        \put(20,-2){\textbf{Number of Time Steps}}
      \end{overpic}
      & \qquad
      %%beta =1
      \begin{overpic}[width=.475\textwidth]{./figures/Energygrowth.eps}
        \put(20,-2){\textbf{Number Of Time Steps}}
      \end{overpic}
      \\[1.5em]
     \end{tabular}
  \end{center}
  \label{fig:EnergyEstimates}
  \caption{Energy Plots against number of time steps. The initial data that yields the plot in the left is that associated with $C = 0.1$ and time step $\Dt=0.001$, whereas the results on the right figure are associated with $C = 5$ and $\Dt=0.21$}
\end{figure}
%
 \subsection{Hartmann Flow}
%%
Consider a square duct of infinite length  containing a conducting fluid.
%
Further assume that this fluid is subjected to a magnetic field that runs along a direction perpendicular to the duct. 
%
This is the set up for the Hartmann Flow problem which is regarded as a benchmark in MHD.
%
The behavior of the fluid will depend on the ratio of the Laplace force and the viscous forces, a dimensionless quantity that goes by the name of Hartmann number. 
%
There are a set of known formulas the describe the solution to this problem, a proof of which can be found in \cite{moreau2013magnetohydrodynamics}.
%
It is for this reason that researchers use the Hartmann flow problem to test the performance of their simulations, see \cite{hu2017stable,codina2006stabilized,shadid2016scalable}.

In this section we consider the computational domain $[-1,1]^2$ as cross section of the aforementioned duct and consider a fluid with conductivity $1$ filling this duct.
%
The magnetic field is applied in the direction of the $y-$axis.
%
If we consider the case where the viscous forces and Laplace forces are of equal strength, so that the Hartmann number is $1$.
%
Then, we can expect the fluid to behave in accordance to $\Bv = (B_x,1,0)$, $\uv=(u_x,0,0)$ and $\Ev = (0,0,E_z)$ for
\begin{equation}
    \begin{aligned}
    &u_x(x,y) = \frac{\cosh{1/2}-\cosh{y}}{2\sinh{1/2}},\\
    &B_x(x,y) = \frac{\sinh{y}-2y\sinh{1/2}}{2\sinh{1/2}},\\
    &E_z(x,y) = \frac{2\sinh{1/2}-\cosh{1/2}}{2\sinh{1/2}}\approx -0.0820.
    \end{aligned}
\end{equation}
%
Note that the $y-$component of the magnetic field is $1$ simply because this was the assumption.
%
Therefore, our main interest in this section is in checking if we can recover approximations to the $x-$component.
%
To do this we feed the analytical solution for the initial and boundary conditions and evolve the system until $T = 10$ with step size $\Dt =0.005$.
\begin{figure}[H]
  \begin{center}
    \begin{tabular}{cc}
      %% Triangular Mesh
      \begin{overpic}[width=.45\textwidth]{./figures/TopNumericalBx.eps}
        \put(35,-2){ { \textbf{x -axis} } }
        \put(-5,35){ 
        \begin{sideways}
        {\textbf{y-axis}} \end{sideways} 
        }
      \end{overpic}
      & \qquad
      %%Quadrilateral Mesh
      \begin{overpic}[width=.45\textwidth]{./figures/SidewaysExactAndNumerical.eps}
        \put(45,-2){{\textbf{y-axis}}}
        \put( -5,35){\begin{sideways}{\textbf{z-axis}}\end{sideways}}
      \end{overpic}
     \end{tabular}
  \end{center}
  \caption{Plots of the numerical and analytic solutions for the $x-$component of the magnetic field, computed in a Voronoi tesselation of mesh size 0.017 using the elliptic projector as the alternative to the mass matrix. The figure on the left is of the numerical solution as viewed from above, whereas the picture on the right shows the numerical solution in a rainbow colorbar overlaid with the exact solution in bold black, both are viewed from the side.}
  \label{fig:HartmannSol}
\end{figure}

The results, to the naked, eye are satisfactory, figure~\ref{fig:HartmannSol} gives evidence of this fact.
%
We further conducted a convergence test that verfies that every alternative to the mass matrix yields a close approximation and provides additional evidence that rate of convergence of the magnetic field is linear, these results are in figure~\ref{fig:HartamnnConvergencePlots}.
%
%%
\begin{figure}[H]
  \begin{center}
    \begin{tabular}{ccc}
      %% Triangular Mesh
      \begin{overpic}[width=.3\textwidth]{./figures/HMagneticTriangularConvergence.eps}
        \put(30,-2){ { \small\textbf{Mesh Size h} } }
        \put( -5,15){ 
        \begin{sideways}
        {\small\textbf{RelativeError}} \end{sideways} 
        }
        \put(15,28){{\small 1}}
        \put(24,35){{\small 1}}
      \end{overpic}
      & \qquad
      %%Quadrilateral Mesh
      \begin{overpic}[width=.3\textwidth]{./figures/HMagneticQuadConvergence.eps}
        \put(30,-2){{\small\textbf{Mesh Size h}}}
        \put( -5,15){\begin{sideways}{\small\textbf{Relative Error}}\end{sideways}}
        \put(15,40){{\small 1}}
        \put(24,46){{\small 1}}
      \end{overpic}
      &\qquad
      %%Voronoi Mesh
      \begin{overpic}[width=.3\textwidth]{./figures/HMagneticVoronoiConvergence.eps}
        \put(30,-2){{\small\textbf{Mesh Size h}}}
        \put(-5,15){\begin{sideways}{\small\textbf{Relative Error}}\end{sideways}}
        \put(13.5,40){{\small 1}}
        \put(22,46){{\small 1}}
      \end{overpic}
     \end{tabular}
  \end{center}
  \caption{Convergence plots for the approximation of the magnetic field on the three different mesh families. The symbols E,LS,GI refers to the three alternatives we have for constructing the nodal mass matrix the elliptic projector, least squares projector and the Galerkin interpolator respectively.}
\label{fig:HartamnnConvergencePlots}
\end{figure}
